JEEM: Vision-Language Understanding in Four Arabic Dialects

We introduce JEEM, a benchmark designed to evaluate Vision-Language Models (VLMs) on visual understanding across four Arabic-speaking countries: Jordan, The Emirates, Egypt, and Morocco. JEEM includes the tasks of image captioning and visual question answering, and features culturally rich and regionally diverse content. This dataset aims to assess the ability of VLMs to generalize across dialects and accurately interpret cultural elements in visual contexts. In an evaluation of five prominent open-source Arabic VLMs and GPT-4V, we find that the Arabic VLMs consistently underperform, struggling with both visual understanding and dialect-specific generation. While GPT-4V ranks best in this comparison, the model's linguistic competence varies across dialects, and its visual understanding capabilities lag behind. This underscores the need for more inclusive models and the value of culturally-diverse evaluation paradigms.

==> Answer.tex <==


\begin{longtable}{|c|c|c|c|c|}
\hline
\textbf{Dialect} & \textbf{Unique Words} & \textbf{Average Length} & \textbf{Top 10 Words} \\
\hline
\endfirsthead
\hline
\textbf{Dialect} & \textbf{Unique Words} & \textbf{Average Length} & \textbf{Top 10 Words} \\
\hline
\endhead
\hline
Jordanian & 9751 & 51.71 & {'أن': 204, 'أو': 240, 'الصورة': 729, 'تظهر': 291, 'على': 747, 'في': 1145, 'من': 836, 'هذه': 335, 'يبدو': 223, 'يظهر': 260} \\
Moroccan & 7087 & 52.96 & {'الصورة': 602, 'بعض': 155, 'تظهر': 201, 'على': 549, 'في': 1184, 'من': 600, 'نرى': 227, 'هذه': 232, 'يبدو': 216, 'يظهر': 278} \\
Egyptian & 11718 & 63.51 & {'إلى': 275, 'الصورة': 765, 'توجد': 297, 'صورة': 281, 'على': 1282, 'في': 1410, 'من': 1527, 'وفي': 234, 'يظهر': 322, 'يوجد': 276} \\
UAE & 1146 & 42.17 & {'أرى': 19, 'أن': 34, 'الإمارات': 20, 'الصورة': 49, 'توجد': 24, 'على': 32, 'في': 88, 'من': 61, 'نرى': 17, 'يرتدي': 18} \\
\hline
\end{longtable}


==> Dialect.tex <==

\begin{longtable}{|c|c|c|c|c|}
\hline
\textbf{Dialect} & \textbf{Unique Words} & \textbf{Average Length} & \textbf{Top 10 Words} \\
\hline
\endfirsthead
\hline
\textbf{Dialect} & \textbf{Unique Words} & \textbf{Average Length} & \textbf{Top 10 Words} \\
\hline
\endhead
\hline
Jordanian & 8933 & 46.40 & {'الصورة': 443, 'اللي': 185, 'على': 557, 'في': 832, 'فيه': 189, 'فيها': 173, 'مبين': 373, 'من': 541, 'هاي': 230, 'وفي': 284} \\
Moroccan & 6780 & 52.90 & {'الصورة': 226, 'ديال': 962, 'شي': 421, 'على': 292, 'في': 279, 'فيها': 238, 'كيبان': 408, 'لي': 268, 'من': 283, 'واحد': 573} \\
Egyptian & 9764 & 58.75 & {'الصورة': 700, 'اللي': 294, 'صورة': 273, 'على': 1147, 'عليها': 247, 'في': 1723, 'فيها': 259, 'كتير': 243, 'من': 1083, 'وفي': 401} \\
UAE & 1083 & 38.87 & {'أشوف': 16, 'الصورة': 35, 'الصوره': 20, 'اللي': 13, 'شيء': 28, 'على': 21, 'في': 101, 'لابس': 14, 'من': 31, 'نشوف': 16} \\
\hline
\end{longtable}

==> automatic_evaluation_captions.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|cccc}

\toprule

 &\textbf{Model} & \textbf{BLEU} & \textbf{CIDEr} & \textbf{ROUGE} & \textbf{BERTSc} \\

\midrule
\multirow{4}{*}{\rotatebox{90}{\textbf{MSA}}}  
& Peacock &  & 1.52 & 7.94 & 79.57 \\  
& Maya & 3.89 & 2.34 & 8.07 & 60.62 \\  
& AIN & 1.91 & 1.91 & 9.76 & 83.49 \\  
& Palo &  &  &  &  \\  
& GPT-4 &  & 7.96 & 11.04 & 82.81 \\  

\midrule
\multirow{4}{*}{\rotatebox{90}{\jordanflag \textbf{JO}}}  
& Peacock & 1.88 & 2.09 & 6.44 & 65.91 \\  
& Maya & 2.16 & 0.82 & 6.82 & 77.65 \\  
& AIN & 1.88 & 0.85 & 5.18 & 70.80 \\  
& Palo & 2.32 & 0.68 & 6.95 & 78.74 \\  
& GPT-4 & 4.89 & 6.81 & 9.79 & 73.00 \\  

\midrule
\multirow{4}{*}{\rotatebox{90}{\uaeflag \textbf{AE}}}  
& Peacock &  &  &  &  \\  
& Maya & 1.52 & 0.17 & 5.98 & 78.76 \\  
& AIN & 1.60 & 0.38 & 5.25 & 60.15 \\  
& Palo &  &  &  &  \\  
& GPT-4 & 2.54 & 2.79 & 6.40 & 79.52 \\  

\midrule
\multirow{4}{*}{\rotatebox{90}{\egyptflag \textbf{EG}}}
& Peacock & 1.06 & 1.34 & 4.74 & 83.86 \\  
& Maya & 1.81 & 0.40 & 6.47 & 88.05 \\  
& AIN & 1.88 & 0.85 & 5.18 & 70.80 \\ 
& Palo & 2.05 & 0.48 & 6.81 & 88.91 \\  
& GPT-4 & 4.09 & 8.41 & 8.56 & 89.74 \\  

\midrule
\multirow{4}{*}{\rotatebox{90}{\moroccoflag \textbf{MA}}}
& Peacock & 0.48 & 0.97 & 2.33 & 46.25 \\  
& Maya & 0.76 & 0.74 & 3.10 & 64.86 \\  
& AIN & 1.00 & 1.42 & 3.13 & 59.70 \\  
& Palo & 0.87 & 0.72 & 2.99 & 65.71 \\  
& GPT-4 & 3.58 & 5.94 & 7.55 & 61.57 \\  

\bottomrule

\end{tabular}
}
\caption{Automatic evaluation of \textbf{image captioning} across different Arabic varieties. Results are shown as percentages.}
\label{tab:automatic_eval}
\end{table}


==> automatic_evaluation_vqa.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}

\toprule
& \jordanflag \textbf{JO} & \uaeflag \textbf{AE} & \egyptflag \textbf{EG} & \moroccoflag \textbf{MA} \\

\midrule
Peacock & 44.96 &  & 47.04 & 52.73 \\
Maya & 52.41 &  & 51.41 & 59.27 \\
AIN & \\
GPT-4 & 54.52 &  & 51.22 & 61.21 \\

\bottomrule

\end{tabular}}
\caption{BERTScore evaluation of \textbf{question answering} results for different Arabic dialects. Results are reported as percentages.}
\label{tab:vqa_bertscore_eval}
\end{table}


==> topics_groups.tex <==

\begin{table}[h] 
    \vspace{0.1cm}
    \centering
    \scriptsize
    \begin{tabular}{lr}
    \toprule 
        \multicolumn{2}{c}{\textbf{أماكن}} \\
        \begin{arabtext} شارع \end{arabtext} & \\
        \begin{arabtext} زقاق \end{arabtext} & \\
        \begin{arabtext} سوق تقليدي \end{arabtext} & \\
        \begin{arabtext} مسجد \end{arabtext} & \\
        \begin{arabtext} مدينة قديمة \end{arabtext} & \\
        \begin{arabtext} محطة قطار \end{arabtext} & \\
        \begin{arabtext} مدينة مغربية \end{arabtext} & \\
        \begin{arabtext} الصحراء \end{arabtext} & \\
        \begin{arabtext} ساحة \end{arabtext} & \\
        \begin{arabtext} قطار \end{arabtext} & \\
        \begin{arabtext} جامع الفنا \end{arabtext} & \\
        \begin{arabtext} قرية مغربية \end{arabtext} & \\
        \begin{arabtext} شفشاون \end{arabtext} & \\
        \begin{arabtext} سوق شعبي \end{arabtext} & \\
        \begin{arabtext} سوق مغربي \end{arabtext} & \\
        \begin{arabtext} المغرب \end{arabtext} & \\
        \begin{arabtext} حديقة \end{arabtext} & \\
        \begin{arabtext} محطة القطار \end{arabtext} & \\
        \begin{arabtext} طريق \end{arabtext} & \\
        \begin{arabtext} كورنيش البحر \end{arabtext} & \\
        \begin{arabtext} مدينة ألعاب \end{arabtext} & \\
        \begin{arabtext} مدينة طنجة \end{arabtext} & \\
        \begin{arabtext} مدينة مراكش \end{arabtext} & \\
        \begin{arabtext} مدينة الصويرة \end{arabtext} & \\
        \begin{arabtext} مدينة صغيرة في جنوب المغرب \end{arabtext} & \\
        \begin{arabtext} قرية \end{arabtext} & \\
        \begin{arabtext} قرية جبلية \end{arabtext} & \\
        \begin{arabtext} قرية صحراوية \end{arabtext} & \\
        \begin{arabtext} مدينة ساحلية \end{arabtext} & \\
        \begin{arabtext} حي المدينة \end{arabtext} & \\
        \begin{arabtext} حي شعبي مغربي \end{arabtext} & \\
        \begin{arabtext} منطقة قروية \end{arabtext} & \\
        \begin{arabtext} منطقة سكنية شعبية \end{arabtext} & \\
        \begin{arabtext} منطقة جبلية \end{arabtext} & \\
        \begin{arabtext} محطة حافلات \end{arabtext} & \\
        \begin{arabtext} محطة ترامواي \end{arabtext} & \\
        \begin{arabtext} محطة سيارات الأجرة \end{arabtext} & \\
        \begin{arabtext} مطار \end{arabtext} & \\
        \begin{arabtext} ميناء \end{arabtext} & \\
        \begin{arabtext} مركز تجاري \end{arabtext} & \\
        \begin{arabtext} مركز الخدمات الطبية \end{arabtext} & \\
        \begin{arabtext} مكتبة الجامعة \end{arabtext} & \\
        \begin{arabtext} مقبرة \end{arabtext} & \\
        \begin{arabtext} مبنى حكومي \end{arabtext} & \\
        \begin{arabtext} مبنى البريد \end{arabtext} & \\
        \begin{arabtext} محطة وقود \end{arabtext} & \\
        \begin{arabtext} سوق مغطى \end{arabtext} & \\
        \begin{arabtext} سوق تقليدي مغربي \end{arabtext} & \\
        \begin{arabtext} سوق سياحي \end{arabtext} & \\
        \begin{arabtext} سوق شعبي مغربي \end{arabtext} & \\
        \begin{arabtext} سوق الملابس \end{arabtext} & \\
        \begin{arabtext} سوق الفواكه والخضروات \end{arabtext} & \\
        \begin{arabtext} سوق الخضار والفواكه \end{arabtext} & \\
        \begin{arabtext} سوق الحبوب \end{arabtext} & \\
        \begin{arabtext} سوق السمك \end{arabtext} & \\
        \begin{arabtext} سوق الأغنام \end{arabtext} & \\
        \begin{arabtext} سوق الماشية \end{arabtext} & \\
        \begin{arabtext} سوق الفواكه \end{arabtext} & \\
        \begin{arabtext} سوق الحبوس \end{arabtext} & \\
        \midrule
        \multicolumn{2}{c}{\textbf{\begin{arabtext} أحداث واحتفالات \end{arabtext}}} \\
        \begin{arabtext} عيد الميلاد \end{arabtext} & \\
        \begin{arabtext} احتفال \end{arabtext} & \\
        \begin{arabtext} احتفال في دبي \end{arabtext} & \\
        \begin{arabtext} حفل زفاف \end{arabtext} & \\
        \begin{arabtext} حفل توزيع الجوائز \end{arabtext} & \\
        \begin{arabtext} مناسبة احتفالية \end{arabtext} & \\
        \begin{arabtext} مهرجان \end{arabtext} & \\
        \begin{arabtext} مهرجان فولكلوري \end{arabtext} & \\
        \begin{arabtext} اجتماع \end{arabtext} & \\
        \begin{arabtext} اجتماع رسمي \end{arabtext} & \\
        \begin{arabtext} ندوة \end{arabtext} & \\
        \begin{arabtext} محاضرة \end{arabtext} & \\
        \begin{arabtext} عرض موسيقي \end{arabtext} & \\
        \begin{arabtext} عرض تقديمي \end{arabtext} & \\
        \begin{arabtext} تظاهرة \end{arabtext} & \\
        \begin{arabtext} فعالية في أغادير \end{arabtext} & \\
        \begin{arabtext} حملة توعية \end{arabtext} & \\
        \begin{arabtext} حملة تطوعية \end{arabtext} & \\
    \midrule
    \bottomrule
    \end{tabular}
    \caption{Topic categories}
    \label{tab:categories_topic}
\end{table}


==> unused_gpt_evaluation_vqa.tex <==
\input{gpt_evaluation_qa}

\paragraph{GPT-Based Evaluation of Question Answering}
We use GPT-4 to assess model-generated answers based on the same criteria used for image captioning: \textbf{Consistency}, \textbf{Relevance}, \textbf{Fluency}, and \textbf{Dialect Authenticity}. Unlike traditional automatic metrics, GPT-4 can incorporate contextual understanding and linguistic nuances into its assessment.

As in image captioning, GPT-4o was used for answer generation, while GPT-4 was used for evaluation. While BERTScore provides a useful semantic similarity measure, it relies solely on the reference answer and does not account for multiple valid responses that may arise based on the image. To address this limitation, we conduct a GPT-based evaluation that considers both the image and the reference answer, allowing for a more context-aware assessment.

In this evaluation, GPT-4 is provided with both the image and the reference answer and is prompted to assess the generated answer according to the four defined criteria. This approach ensures that responses are evaluated not just based on lexical similarity but also on their alignment with the visual context. The results of this evaluation are presented in \autoref{tab:gpt_eval_qa}.

The prompts used for GPT-based evaluation are detailed in \autoref{sec:eval_prompts}.
